MPCLeague: Robust MPC Platform for Privacy-Preserving Machine Learning

In the modern era of computing, machine learning tools have demonstrated their potential in vital sectors, such as healthcare and finance, to derive proper inferences. The sensitive and confidential nature of the data in such sectors raises genuine concerns for data privacy. This motivated the area of Privacy-preserving Machine Learning (PPML), where privacy of data is guaranteed. In this thesis, we design an efficient platform, MPCLeague, for PPML in the Secure Outsourced Computation (SOC) setting using Secure Multi-party Computation (MPC) techniques. MPC, the holy-grail problem of secure distributed computing, enables a set of n mutually distrusting parties to perform joint computation on their private inputs in a way that no coalition of t parties can learn more information than the output (privacy) or affect the true output of the computation (correctness). While MPC, in general, has been a subject of extensive research, the area of MPC with a small number of parties has drawn popularity of late mainly due to its application to real-time scenarios, efficiency and simplicity. This thesis focuses on designing efficient MPC frameworks for 2, 3 and 4 parties, with at most one corruption and supports ring structures. At the heart of this thesis are four frameworks - ASTRA, SWIFT, Tetrad, ABY2.0 - catered to different settings. The practicality of our framework is argued through improvements in the benchmarking of widely used ML algorithms -- Linear Regression, Logistic Regression, Neural Networks, and Support Vector Machines. We propose two variants for each of our frameworks, with one variant aiming to minimise the execution time while the other focuses on the monetary cost. The concrete efficiency gains of our frameworks coupled with the stronger security guarantee of robustness make our platform an ideal choice for a real-time deployment of PPML techniques.

==> bench2pcS/Bench_InfPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
		\resizebox{.37\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=6000,
					xtick={1,2,3}, xticklabels={SVM,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.28,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-13pt,hide axis, legend style = {at={(0.82, 0.85)}}]
					\addplot+ coordinates
					{(1,898.8) (2,1065.35) (3,326.46)}; 	
					\addlegendentry{{\footnotesize SecureML}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.82, 0.775)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,5271.74) (2,5882.44) (3,934.34)}; 	
					\addlegendentry{{\footnotesize \TWthisT~~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=13pt, legend style = {at={(0.82, 0.7)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,3221.29) (2,3746.89) (3,891.19)};  
					\addlegendentry{\footnotesize \TWthisC~~}
				\end{axis}
				
			\end{tikzpicture}
		}
%	\vspace{-1mm}
	\caption{Inference of SVM, NN-3 and NN-4: in terms of $\TP$ (higher is better)}\label{fig:MLTP2pcS}
	%\vspace{-2mm}
\end{figure}

==> bench2pcS/Bench_TrainPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
	\begin{subfigure}{.37\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=75,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,8.06) (2,8.13) (3,21.79) (4,72.01)}; 	
					\addlegendentry{{\footnotesize SecureML~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,1.93) (2,2.05) (3,5.67) (4,25.90)}; 	
					\addlegendentry{{\footnotesize \TWthisT~~~~~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,2.55) (2,2.67) (3,8.40) (4,38.35)};  
					\addlegendentry{\footnotesize \TWthisC~~~~~}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Online Execution Time~(${\sf PT}_{\sf on}$)}\label{fig:TrainA2pcS}
	\end{subfigure}
    %-----------------------------------------
    \hspace{2mm}
	%-----------------------------------------
	\begin{subfigure}{.37\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=650,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4\footnote{scaled down by a factor of $10$}},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,49.33) (2,70) (3,331.01) (4,577.927)}; 	
					\addlegendentry{{\footnotesize SecureML~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,58.51) (2,75.67) (3,343.73) (4,514.610)}; 	
					\addlegendentry{{\footnotesize \TWthisT~~~~~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,34.29) (2,49.16) (3,240.41) (4,399.930)};  
					\addlegendentry{\footnotesize \TWthisC~~~~~}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Monetary Cost~(${\sf Cost}$)}\label{fig:TrainC2pcS}
	\end{subfigure}
	%-----------------------------------------
	\vspace{-1mm}
	\caption{Training of Neural Networks: in terms of ${\sf PT}_{\sf on}$  and ${\sf Cost}$ (lower is better)}\label{fig:MLTrain2pcS}
	%\vspace{-4mm}
\end{figure}

==> bench3pcM/Bench_InfPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
		\resizebox{.37\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=6000,
					xtick={1,2,3}, xticklabels={SVM,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.28,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-13pt,hide axis, legend style = {at={(0.82, 0.85)}}]
					\addplot+ coordinates
					{(1,898.8) (2,1065.35) (3,326.46)}; 	
					\addlegendentry{{\footnotesize Trident~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.82, 0.775)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,5271.74) (2,5882.44) (3,934.34)}; 	
					\addlegendentry{{\footnotesize \FthisT~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=13pt, legend style = {at={(0.82, 0.7)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,3221.29) (2,3746.89) (3,891.19)};  
					\addlegendentry{\footnotesize \FthisC~}
				\end{axis}
				
				% and bar shift +10pt here
			    \begin{axis}[bar shift=26pt, legend style = {at={(0.82, 0.625)}}]
			    	\addplot+[fill=UniBlau] coordinates
			    	{(1,2949.76) (2,3384.51) (3,891.19)}; 		
			    	\addlegendentry{\footnotesize SWIFT~~}
			    \end{axis}
			
			\end{tikzpicture}
		}
%	\vspace{-1mm}
	\caption{Inference of SVM, NN-3 and NN-4: in terms of $\TP$ (higher is better)}\label{fig:MLTP4pcM}
	%\vspace{-2mm}
\end{figure}

==> bench3pcM/Bench_TrainPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
	\begin{subfigure}{.37\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=75,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,8.06) (2,8.13) (3,21.79) (4,72.01)}; 	
					\addlegendentry{{\footnotesize Trident~~~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,1.93) (2,2.05) (3,5.67) (4,25.90)}; 	
					\addlegendentry{{\footnotesize \FthisT~~~~~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,2.55) (2,2.67) (3,8.40) (4,38.35)};  
					\addlegendentry{\footnotesize \FthisC~~~~~}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Online Execution Time~(${\sf PT}_{\sf on}$)}\label{fig:TrainA4pcM}
	\end{subfigure}
    %-----------------------------------------
    \hspace{2mm}
	%-----------------------------------------
	\begin{subfigure}{.37\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=650,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4\footnote{scaled down by a factor of $10$}},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,49.33) (2,70) (3,331.01) (4,577.927)}; 	
					\addlegendentry{{\footnotesize Trident~~~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,58.51) (2,75.67) (3,343.73) (4,514.610)}; 	
					\addlegendentry{{\footnotesize \FthisT~~~~~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,34.29) (2,49.16) (3,240.41) (4,399.930)};  
					\addlegendentry{\footnotesize \FthisC~~~~~}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Monetary Cost~(${\sf Cost}$)}\label{fig:TrainC4pcM}
	\end{subfigure}
	%-----------------------------------------
	\vspace{-1mm}
	\caption{Training of Neural Networks: in terms of ${\sf PT}_{\sf on}$  and ${\sf Cost}$ (lower is better)}\label{fig:MLTrain4pcM}
	%\vspace{-4mm}
\end{figure}

==> bench3pcS/Bench_InfPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
		\resizebox{.37\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=6000,
					xtick={1,2,3}, xticklabels={SVM,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.28,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-13pt,hide axis, legend style = {at={(0.82, 0.85)}}]
					\addplot+ coordinates
					{(1,898.8) (2,1065.35) (3,326.46)}; 	
					\addlegendentry{{\footnotesize ABY3~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.82, 0.775)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,5271.74) (2,5882.44) (3,934.34)}; 	
					\addlegendentry{{\footnotesize \TSthisT}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=13pt, legend style = {at={(0.82, 0.7)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,3221.29) (2,3746.89) (3,891.19)};  
					\addlegendentry{\footnotesize \TSthisC}
				\end{axis}
				
			
			\end{tikzpicture}
		}
%	\vspace{-1mm}
	\caption{Inference of SVM, NN-3 and NN-4: in terms of $\TP$ (higher is better)}\label{fig:MLTP3pcS}
	%\vspace{-2mm}
\end{figure}

==> bench3pcS/Bench_TrainPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
	\begin{subfigure}{.32\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=140,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,5.66) (2,5.78) (3,18.58) (4,134.63)}; 	
					\addlegendentry{{\footnotesize ABY3~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,1.55) (2,1.64) (3,5.42) (4,49.72)}; 	
					\addlegendentry{{\footnotesize \TSthisT}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,2.17) (2,2.26) (3,8.15) (4,66.54)};  
					\addlegendentry{\footnotesize \TSthisC}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Training: ${\sf PT}_{\sf on}$}\label{fig:TrainA3pcS}
	\end{subfigure}
    %-----------------------------------------
 %   \hspace{1mm}
	%-----------------------------------------
	\begin{subfigure}{.32\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=650,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,48.49) (2,115.65) (3,642.07) (4,17134.85)}; 	
					\addlegendentry{{\footnotesize ABY3~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,58.51) (2,75.67) (3,343.73) (4,514.610)}; 	
					\addlegendentry{{\footnotesize \TSthisT}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,34.29) (2,49.16) (3,240.41) (4,399.930)};  
					\addlegendentry{\footnotesize \TSthisC}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Training: ${\sf Cost}$}\label{fig:TrainB3pcS}
	\end{subfigure}
	%-----------------------------------------
	 %-----------------------------------------
%	\hspace{1mm}
	%-----------------------------------------
	\begin{subfigure}{.32\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=6000,
					xtick={1,2,3}, xticklabels={SVM,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.28,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-13pt,hide axis, legend style = {at={(0.82, 0.85)}}]
					\addplot+ coordinates
					{(1,898.8) (2,1065.35) (3,326.46)}; 	
					\addlegendentry{{\footnotesize ABY3~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.82, 0.775)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,5271.74) (2,5882.44) (3,934.34)}; 	
					\addlegendentry{{\footnotesize \TSthisT}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=13pt, legend style = {at={(0.82, 0.7)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,3221.29) (2,3746.89) (3,891.19)};  
					\addlegendentry{\footnotesize \TSthisC}
				\end{axis}
				
				
			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Inference: $\TP$}\label{fig:Inf3pcS}
	\end{subfigure}
	%-----------------------------------------
	\vspace{-1mm}
	\caption{Analysis of protocols in terms of ${\sf PT}_{\sf on}$, ${\sf Cost}$ and $\TP$. The values for NN-4 in  scaled down by a factor of $10$.}\label{fig:MLPlot3pcS}
	%\vspace{-4mm}
\end{figure}

==> bench4pcM/Bench_InfPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
		\resizebox{.37\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=6000,
					xtick={1,2,3}, xticklabels={SVM,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.28,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-13pt,hide axis, legend style = {at={(0.82, 0.85)}}]
					\addplot+ coordinates
					{(1,898.8) (2,1065.35) (3,326.46)}; 	
					\addlegendentry{{\footnotesize Trident~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.82, 0.775)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,5271.74) (2,5882.44) (3,934.34)}; 	
					\addlegendentry{{\footnotesize \FthisT~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=13pt, legend style = {at={(0.82, 0.7)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,3221.29) (2,3746.89) (3,891.19)};  
					\addlegendentry{\footnotesize \FthisC~}
				\end{axis}
				
				% and bar shift +10pt here
			    \begin{axis}[bar shift=26pt, legend style = {at={(0.82, 0.625)}}]
			    	\addplot+[fill=UniBlau] coordinates
			    	{(1,2949.76) (2,3384.51) (3,891.19)}; 		
			    	\addlegendentry{\footnotesize SWIFT~~}
			    \end{axis}
			
			\end{tikzpicture}
		}
%	\vspace{-1mm}
	\caption{Inference of SVM, NN-3 and NN-4: in terms of $\TP$ (higher is better)}\label{fig:MLTP4pcM}
	%\vspace{-2mm}
\end{figure}

==> bench4pcM/Bench_TrainPlot.tex <==
%------------------Full Width Attempt-----------------------------------------------------------
\begin{figure}[htb!]
	\centering
	%-------------------------------------------------
	\begin{subfigure}{.37\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=75,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,8.06) (2,8.13) (3,21.79) (4,72.01)}; 	
					\addlegendentry{{\footnotesize Trident~~~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,1.93) (2,2.05) (3,5.67) (4,25.90)}; 	
					\addlegendentry{{\footnotesize \FthisT~~~~~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,2.55) (2,2.67) (3,8.40) (4,38.35)};  
					\addlegendentry{\footnotesize \FthisC~~~~~}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Online Execution Time~(${\sf PT}_{\sf on}$)}\label{fig:TrainA4pcM}
	\end{subfigure}
    %-----------------------------------------
    \hspace{2mm}
	%-----------------------------------------
	\begin{subfigure}{.37\textwidth}
		\centering
		\resizebox{.95\textwidth}{!}{
			\begin{tikzpicture}[
				every axis/.style={ % add these settings to all the axis environments in the tikzpicture
					ybar stacked,
					ymin=0,ymax=650,
					xtick={1,2,3,4}, xticklabels={NN-1,NN-2,NN-3,NN-4\footnote{scaled down by a factor of $10$}},
					%xlabel={Network}, 
					%ylabel={Online RunTime},
					enlarge x limits=0.2,
					%symbolic x coords={1,2},
					cycle list name=exotic, 
					every axis plot/.append style={fill,draw=none,no markers},
					%nodes near coords, 
					legend style = {anchor = south, legend columns = -1, draw=none, area legend},
					bar width=10pt},]
				
				\begin{axis}[bar shift=-12pt,hide axis, legend style = {at={(0.2, 0.825)}}]
					\addplot+ coordinates
					{(1,49.33) (2,70) (3,331.01) (4,577.927)}; 	
					\addlegendentry{{\footnotesize Trident~~~~~~}}
				\end{axis}
				
				% zero bar shift here    
				\begin{axis}[hide axis, legend style = {at={(0.2, 0.75)}}]
					\addplot+[fill=UniOrange] coordinates
					{(1,58.51) (2,75.67) (3,343.73) (4,514.610)}; 	
					\addlegendentry{{\footnotesize \FthisT~~~~~}}
				\end{axis}
				
				% and bar shift +10pt here
				\begin{axis}[bar shift=12pt, legend style = {at={(0.2, 0.675)}}]
					\addplot+[fill=UniGruen] coordinates
					{(1,34.29) (2,49.16) (3,240.41) (4,399.930)};  
					\addlegendentry{\footnotesize \FthisC~~~~~}
				\end{axis}

			\end{tikzpicture}
		}
		\vspace{-1mm}
		\caption{\footnotesize Monetary Cost~(${\sf Cost}$)}\label{fig:TrainC4pcM}
	\end{subfigure}
	%-----------------------------------------
	\vspace{-1mm}
	\caption{Training of Neural Networks: in terms of ${\sf PT}_{\sf on}$  and ${\sf Cost}$ (lower is better)}\label{fig:MLTrain4pcM}
	%\vspace{-4mm}
\end{figure}

==> chap_MLalgorithms.tex <==





%-----------------------------------------
\subsection{Secure Training}
\label{sec:Bench_Training}
%-----------------------------------------
The training phase in most of the machine learning algorithms consists of two stages-- i) forward propagation, where the model computes the output, and ii) backward propagation, where the model parameters are adjusted according to the computed output and the actual output. We define one {\em iteration} in the training phase as one forward propagation followed by a backward propagation.




%----------------------------------------
\section{Linear Regression}
\label{sec:linreg}
%----------------------------------------
For linear regression, one iteration can be viewed as updating the weight vector $\vecW$ using the Gradient Descent algorithm (GD). The update function for $\vecW$ is given by
%---------------
\begin{align*}
	\vecW = \vecW - \frac{\alpha}{B} \Mat{X}_i^{T}  \circ (\Mat{X}_i \circ \vecW-\Mat{Y}_i)
\end{align*}
%---------------
where $\alpha$ denotes the learning rate and $\Mat{X}_i$ denotes a subset of batch size $B$, randomly selected from the entire dataset in the $i$th iteration. Here the forward propagation consists of computing $\Mat{X}_i \circ \vecW$, while the weight vector is updated in the backward propagation. The update function consists of a series of matrix multiplications, which in turn can be achieved using dot product protocols. The operations of subtraction as well as multiplication by a public constant can be performed locally. We observe that the aforementioned update function can be computed entirely in the arithmetic domain and can be viewed in form of $\shrd$-shares as
%---------------
\begin{align*}
	\shr{\vecW} = \shr{\vecW} - \frac{\alpha}{B} \shr{\Mat{X}_j^{T}}  \circ (\shr{\Mat{X}_j} \circ \shr{\vecW}-\shr{\Mat{Y}_j})
\end{align*}


%----------------------------------------
\section{Logistic Regression}
\label{sec:logreg}
%----------------------------------------

The iteration for the case of logistic regression is similar to that of linear regression, apart from an activation function being applied on $\Mat{X}_i \circ \vecW$ in the forward propagation. We instantiate the activation function using sigmoid (Section~\ref{sec:actFunc}). The update function for $\vecW$ is given by
%---------------
\begin{align*}
	\vecW = \vecW - \frac{\alpha}{B} \Mat{X}_i^{T}  \circ \left(\Sig(\Mat{X}_i \circ \vecW)-\Mat{Y}_i\right)
\end{align*}
%---------------
One iteration of logistic regression incurs an additional cost for computing $\Sig(\Mat{X}_j  \circ {\vecW})$ as compared with that for linear regression.


%----------------------------------------
\section{Neural Networks}
\label{sec:neuralnets}
%----------------------------------------
For the case of NN, we follow steps similar to that of ABY3, where each node across all the layers, except the last layer, uses ReLU ($\ReLU$) as the activation function. At the output layer, we use the MPC friendly variant of the softmax activation function, $\mathsf{smx(u_i) = \frac{\ReLU(u_i)}{\sum_{j = 1}^{n_{f}} \ReLU(u_j)}}$, proposed by SecureML~\cite{MohasselZ17}. In order to perform the division, we switch from arithmetic to garbled world and then use a division garbled circuit. 

The network is trained using the Gradient Descent, where the forward propagation comprises of computing activation matrices for all the layers in the network. Here, the activation matrix for all the layers except the output, is defined as $\Mat{A}_i = \ReLU(\Mat{U}_i)$, where $\Mat{U}_i = \Mat{A}_{i-1}  \circ \Mat{W}_i$ . $\Mat{A}_{0}$ is initialized to $\Mat{X}_{j}$, where $\Mat{X}_j$ is a subset of batch size $B$, randomly selected from the entire dataset for the $j^{th}$ iteration. The activation matrix for the output layer is defined as $\Mat{A}_m  = \mathsf{smx(\Mat{U}_m)}$. 

During the backward propagation, error matrices are computed first. The error matrix for the output layer is defined as $\Mat{E}_m = (\Mat{A}_m - \Mat{T})$, while for the remaining layers it is defined as $\Mat{E}_i = (\Mat{E}_{i+1} \circ \Mat{W}_i^T) \otimes \dReLU(\Mat{U}_i)$. Here the operation $\otimes$ denotes element wise multiplication and $\dReLU$ denotes the derivative of ReLU. This is followed by updating the weights as $\Mat{W}_i = \Mat{W}_i - \frac{\alpha}{B} \Mat{A}_{i-1}^T  \circ \Mat{E}_i$. 
